On The Effects Of Data Normalisation For Domain Adaptation On EEG Data

In the Machine Learning (ML) literature, a well-known problem is the Dataset Shift problem where, differently from the ML standard hypothesis, the data in the training and test sets can follow different probability distributions, leading ML systems toward poor generalisation performances. This problem is intensely felt in the Brain-Computer Interface (BCI) context, where bio-signals as Electroencephalographic (EEG) are often used. In fact, EEG signals are highly non-stationary both over time and between different subjects. To overcome this problem, several proposed solutions are based on recent transfer learning approaches such as Domain Adaption (DA). In several cases, however, the actual causes of the improvements remain ambiguous. This paper focuses on the impact of data normalisation, or standardisation strategies applied together with DA methods. In particular, using \textit{SEED}, \textit{DEAP}, and \textit{BCI Competition IV 2a} EEG datasets, we experimentally evaluated the impact of different normalization strategies applied with and without several well-known DA methods, comparing the obtained performances. It results that the choice of the normalisation strategy plays a key role on the classifier performances in DA scenarios, and interestingly, in several cases, the use of only an appropriate normalisation schema outperforms the DA technique.

==> tables/BCIc_CS_GRL_table.tex <==
\begin{table*}[!h]
\centering
\caption{BCIcIV - CROSS-SESSION - DA-end-to-end}
\begin{tabular}{|c|c|c|c|}
    \hline
    Normalization & noDA-ANN & ANN-DANN & ANN-ADDA\\
    \hline
    $no\_norm$ & $57.56 \pm 10.47$ & $55.94 \pm 8.87$ & $54.79 \pm 15.46$\\
    $N_{0}$ & $54.63 \pm 10.32$ & $56.94 \pm 8.63$ & $60.15 \pm 15.85$\\
    $N_{2}$ & $64.97 \pm 14.28$ & $64.12 \pm 15.39$ & $60.15 \pm 15.68$\\
    \hline
\end{tabular}
\label{tab:bcic_cs_grl_results}
\end{table*}

==> tables/BCIc_CS_SVM_table.tex <==
\begin{table*}[!h]
\centering
\caption{BCIcIV - CROSS SESSION - DA-proiettori}
\begin{tabular}{|c|c|c|c|}
    \hline
    Normalization & noDA-SVM+FBCSP & SVM+FBCSP+TCA & SVM+FBCSP+KPCA\\
    \hline
    $no\_norm$ & $55.79 \pm 9.38$ & $50.54 \pm 1.52$ & $55.79 \pm 9.38$\\
    $N_{0}$ & $55.48 \pm 9.62$ & $55.79 \pm 9.63$ & $55.48 \pm 9.62$\\
    $N_{2}$ & $63.43 \pm 15.10$ & $63.66 \pm 15.17$ & $63.43 \pm 15.10$\\
    \hline
\end{tabular}
\label{tab:bcic_cs_svm_results}
\end{table*}

==> tables/BCIc_LOSO_GRL_table.tex <==
\begin{table*}[!h]
\centering
\caption{BCIcIV - LOSO - DA-end-to-end}
\begin{tabular}{|c|c|c|c|}
    \hline
    Normalization & noDA-ANN & ANN+DANN & ANN+ADDA\\
    \hline
    noNorm & $61.42 \pm 13.36$ & $62.19 \pm 13.43$ & $63.22 \pm 12.90$\\
    $N_{0}$ & $62.11 \pm 13.54$ & $61.73 \pm 13.02$ & $62.84 \pm 13.77$\\
    % $N_{1}$ & $61.65 \pm 11.84$ & $62.04 \pm 13.69$ & $62.84 \pm 14.24$\\
    $N_{2}$ & $67.98 \pm 11.81$ & $67.52 \pm 11.40$ & $68.58 \pm 10.96$\\
    % $N_{3}$ & $66.36 \pm 12.18$ & $68.13 \pm 13.87$ & $59.77 \pm 11.14$\\
    \hline
\end{tabular}
\label{tab:bcic_loso_grl_results}
\end{table*}

==> tables/BCIc_LOSO_SVM_table.tex <==
\begin{table*}[!h]
\centering
\caption{BCIcIV - LOSO - DA-proiettori}
\begin{tabular}{|c|c|c|c|}
    \hline
    Normalization & noDA-SVM+FBCSP & SVM+FBCSP+TCA & SVM+FBCSP+KPCA\\
    \hline
    noNorm & $61.03 \pm 12.70$ & $56.10 \pm 10.62$ & $61.11 \pm 12.62$\\
    % $N_{0}$ & $61.11 \pm 13.38$ & $61.03 \pm 12.47$ & $ \pm $\\
    % $N_{1}$ & $61.73 \pm 10.92$ & $59.41 \pm 10.49$ & $ \pm $\\
    $N_{0}$ & $61.11 \pm 12.62$ & $61.03 \pm 11.76$ & $61.11 \pm 12.62$\\
    $N_{2}$ & $68.52 \pm 11.35$ & $67.90 \pm 11.89$ & $68.51 \pm 11.35$\\
    % $N_{3}$ & $67.90 \pm 13.10$ & $67.44 \pm 14.37$ & $ \pm $\\
    \hline
\end{tabular}
\label{tab:bcic_loso_svm_results}
\end{table*}

==> tables/DEAP_LOSO_GRL_table.tex <==
\begin{table*}[!h]
\centering
\caption{DEAP - LOSO - DA-end-to-end}
\begin{tabular}{|c|c|c|c|}
    \hline
    Normalization & noDA-ANN & ANN+DANN & ANN+ADDA\\
    \hline
    noNorm & $34.21 \pm 4.11$ & $34.21 \pm 3.15$ & $33.93 \pm 2.15$\\
    $N_{0}$ & $30.44 \pm 10.13$ & $31.11 \pm 13.38$ & $34.92 \pm 13.64$\\
    $N_{1}$ & $35.60 \pm 8.72$ & $36.51 \pm 7.90$ & $34.92 \pm 13.64$\\
    $N_{2}$ & $36.67 \pm 12.45$ & $35.52 \pm 13.84$ & $32.94 \pm 11.59$\\
    $N_{3}$ & $39.33 \pm 14.08$ & $41.27 \pm 14.91$ & $38.89 \pm 14.16$\\
    \hline
\end{tabular}
\label{tab:deap_loso_grl_results}
\end{table*}

==> tables/DEAP_LOSO_SVM_table.tex <==
\begin{table*}[!h]
\centering
\caption{DEAP - LOSO - DA-proiettori}
\begin{tabular}{|c|c|c|c|}
    \hline
    Normalization & noDA-SVM & SVM+TCA & SVM+KPCA\\
    \hline
    $no\_norm$ & $31.31 \pm 9.76$ & $36.90 \pm 12.34$ & $41.23 \pm 10.02$\\
    $N_{0}$ & $32.56 \pm 1.94$ & $41.23 \pm 13.26$ & $38.33 \pm 9.86$\\
    $N_{1}$ & $32.55 \pm 10.83$ & $42.66 \pm 11.70$ & $34.52 \pm 7.42$\\
    $N_{2}$ & $32.13 \pm 14.77$ & $42.46 \pm 15.99$ & $40.67 \pm 15.13$\\
    $N_{3}$ & $33.73 \pm 14.75$ & $42.62 \pm 17.06$ & $43.77 \pm 12.68$\\
    \hline
\end{tabular}
\label{tab:deap_loso_svm_results}
\end{table*}

==> tables/SEED_CS_GRL_table.tex <==
\begin{table*}[!h]
\centering
\caption{SEED - CROSS-SESSION - DA-end-to-end}
\begin{tabular}{|c|c|c|c|}
    \hline
    Normalization & noDA-ANN & ANN+DANN & ANN+ADDA\\
    \hline
    noNorm & $45.47 \pm 20.43$ & $43.15 \pm 17.43$ & $37.10 \pm 10.83$\\
    $N_{0}$ & $64.85 \pm 17.38$ & $51.76 \pm 17.71$ & $57.33 \pm 19.52$\\
    $N_{1}$ & $66.37 \pm 16.16$ & $55.25 \pm 19.95$ & $65.07 \pm 17.50$\\
    $N_{2}$ & $83.93 \pm 9.60$ & $83.84 \pm 10.55$ & $76.80 \pm 12.50$\\
    $N_{3}$ & $83.09 \pm 9.98$ & $84.43 \pm 9.67$ & $77.80 \pm 12.82$\\
    \hline
\end{tabular}
\label{tab:seed_cs_grl_results}
\end{table*}

==> tables/SEED_CS_SVM_table.tex <==
\begin{table*}[!h]
\centering
\caption{SEED - CROSS SESSION - DA-proiettori}
\begin{tabular}{|c|c|c|c|}
    \hline
    Normalization & noDA-SVM & SVM+TCA & SVM+KPCA\\
    \hline
    noNorm & $63.63 \pm 18.92$ & $47.52 \pm 12.45$ & $61.31 \pm 14.33$\\
    $N_{0}$ & $62.32 \pm 17.33$ & $79.56 \pm 10.21$ & $61.66 \pm 16.88$\\
    $N_{1}$ & $63.39 \pm 20.02$ & $76.96 \pm 12.99$ & $63.25 \pm 15.92$\\
    $N_{2}$ & $85.59 \pm 9.89$ & $81.67 \pm 11.83$ & $83.62 \pm 9.45$\\
    $N_{3}$ & $86.56 \pm 8.15$ & $83.15 \pm 10.92$ & $84.09 \pm 10.45$\\
    \hline
\end{tabular}
\label{tab:seed_cs_svm_results}
\end{table*}

==> tables/SEED_LOSO_GRL_table.tex <==
\begin{table*}[!h]
\centering
\caption{SEED - LOSO - DA-end-to-end}
\begin{tabular}{|c|c|c|c|}
    \hline
    Normalization & noDA-ANN & ANN+DANN & ANN+ADDA\\
    \hline
    noNorm & $45.50 \pm 13.18$ & $50.65 \pm 12.19$ & $33.13 \pm 0.22$\\
    $N_{0}$ & $48.31 \pm 14.09$ & $43.60 \pm 11.86$ & $43.97 \pm 12.86$\\
    $N_{1}$ & $50.54 \pm 15.13$ & $60.35 \pm 21.45$ & $46.53 \pm 12.92$\\
    $N_{2}$ & $81.52 \pm 7.26$ & $79.03 \pm 7.71$ & $70.43 \pm 14.17$\\
    $N_{3}$ & $75.22 \pm 7.85$ & $75.79 \pm 4.78$ & $60.57 \pm 13.92$\\
    \hline
\end{tabular}
\label{tab:seed_loso_grl_results}
\end{table*}

==> tables/SEED_LOSO_SVM_table.tex <==
\begin{table*}[!h]
\centering
\caption{SEED - LOSO - DA-proiettori}
\begin{tabular}{|c|c|c|c|}
    \hline
    Normalization & noDA-SVM & SVM+TCA & SVM+KPCA\\
    \hline
    noNorm & $52.96 \pm 9.82$ & $46.68 \pm 13.34$ & $58.61 \pm 7.50$\\
    $N_{0}$ & $52.47 \pm 11.33$ & $71.58 \pm 7.16$ & $48.16 \pm 13.22$\\
    $N_{1}$ & $52.32 \pm 15.06$ & $79.70 \pm 8.98$ & $53.59 \pm 16.91$\\
    $N_{2}$ & $74.71 \pm 8.47$ & $80.09 \pm 6.51$ & $80.74 \pm 6.11$\\
    $N_{3}$ & $73.24 \pm 8.37$ & $76.37 \pm 7.44$ & $73.91 \pm 7.31$\\
    \hline
\end{tabular}
\label{tab:seed_loso_svm_results}
\end{table*}
